Spatiotemporal Synchronization of Distributed Arrays using Particle-Based Loopy Belief Propagation

Sensing and imaging with distributed radio infrastructures (e.g., distributed MIMO, wireless sensor networks, multistatic radar) rely on knowledge of the positions, orientations, and clock parameters of distributed apertures. We extend a particle-based loopy belief propagation (BP) algorithm to cooperatively synchronize distributed agents to anchors in space and time. Substituting marginalization over nuisance parameters with approximate but closed-form concentration, we derive an efficient estimator that bypasses the need for preliminary channel estimation and operates directly on noisy channel observations. Our algorithm demonstrates scalable, accurate spatiotemporal synchronization on simulated data.

==> IEEEabrv.tex <==
journal = IEEE_J_AC,
@STRING{IEEE_J_ANNE = "{IEEE} Trans. Aeronaut. Navig. Electron."}
@STRING{IEEE_J_AES = "{IEEE} Trans. Aerosp. Electron. Syst."}
@STRING{IEEE_J_ANE = "{IEEE} Trans. Aerosp. Navig. Electron."}
@STRING{IEEE_J_AS = "{IEEE} Trans. Aerosp."}
@STRING{IEEE_J_AIRE = "{IEEE} Trans. Airborne Electron."}
@STRING{IEEE_J_MIL = "{IEEE} Trans. Mil. Electron."}
@STRING{IEEE_J_ITS = "{IEEE} Trans. Intell. Transp. Syst."}
@STRING{IEEE_J_IV = "{IEEE} Trans. Intell. Veh."}
@STRING{IEEE_J_TTE = "{IEEE} Trans. Transport. Electrific."}
@STRING{IEEE_J_VC = "{IEEE} Trans. Veh. Commun."}
@STRING{IEEE_J_VT = "{IEEE} Trans. Veh. Technol."}
@STRING{IEEE_J_STSP = "{IEEE} J. Sel. Topics Signal Process."}
@STRING{IEEE_J_SPL = "{IEEE} Signal Process. Lett."}
@STRING{IEEE_J_SYST = "{IEEE} Syst. J."}
@STRING{IEEE_J_ASSP = "{IEEE} Trans. Acoust., Speech, Signal Process."}
@STRING{IEEE_J_AU = "{IEEE} Trans. Audio"}
@STRING{IEEE_J_AUEA = "{IEEE} Trans. Audio Electroacoust."}
@STRING{IEEE_J_ASLP = "{IEEE/ACM} Trans. Audio, Speech, Language Process."}
@STRING{IEEE_J_ASL = "{IEEE} Audio, Speech, Language Process."}
@STRING{IEEE_J_AC = "{IEEE} Trans. Autom. Control"}
@STRING{IEEE_J_CAS = "{IEEE} Trans. Circuits Syst."}
@STRING{IEEE_J_CASVT = "{IEEE} Trans. Circuits Syst. Video Technol."}
@STRING{IEEE_J_CASI = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CASI_RP = "{IEEE} Trans. Circuits Syst. {I}"}
@STRING{IEEE_J_CASII_EB = "{IEEE} Trans. Circuits Syst. {II}"}
@STRING{IEEE_J_CT = "{IEEE} Trans. Circuit Theory"}
@STRING{IEEE_J_CST = "{IEEE} Trans. Control Syst. Technol."}
@STRING{IEEE_J_ETCAS = "{IEEE} Trans. Emerg. Sel. Topics Circuits Syst."}
@STRING{IEEE_J_SP = "{IEEE} Trans. Signal Process."}
@STRING{IEEE_J_SU = "{IEEE} Trans. Sonics Ultrason."}
@STRING{IEEE_J_SAP = "{IEEE} Trans. Speech Audio Process."}
@STRING{IEEE_J_UE = "{IEEE} Trans. Ultrason. Eng."}
@STRING{IEEE_J_UFFC = "{IEEE} Trans. Ultrason., Ferroelectr., Freq. Control"}
@STRING{IEEE_J_COML = "{IEEE} Commun. Lett."}
@STRING{IEEE_J_JSAC = "{IEEE} J. Sel. Areas Commun."}
@STRING{IEEE_J_COM = "{IEEE} Trans. Commun."}
@STRING{IEEE_J_COMT = "{IEEE} Trans. Commun. Technol."}
@STRING{IEEE_J_WCOM = "{IEEE} Trans. Wireless Commun."}
@STRING{IEEE_J_WCOML = "{IEEE} Wireless Commun. Lett."}
@STRING{IEEE_J_ADVP = "{IEEE} Trans. Adv. Packag."}
@STRING{IEEE_J_CHMT = "{IEEE} Trans. Compon., Hybrids, Manuf. Technol."}
@STRING{IEEE_J_CPMT = "{IEEE} Trans. Compon. Packag. Manuf. Technol."}
@STRING{IEEE_J_CPMTA = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {A}"}
@STRING{IEEE_J_CPMTB = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {B}"}
@STRING{IEEE_J_CPMTC = "{IEEE} Trans. Compon., Packag., Manuf. Technol. {C}"}
@STRING{IEEE_J_CAPTS = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CAPT = "{IEEE} Trans. Compon. Packag. Technol."}
@STRING{IEEE_J_CPART = "{IEEE} Trans. Compon. Parts"}
@STRING{IEEE_J_EPM = "{IEEE} Trans. Electron. Packag. Manuf."}
@STRING{IEEE_J_MFT = "{IEEE} Trans. Manuf. Technol."}
@STRING{IEEE_J_PHP = "{IEEE} Trans. Parts, Hybrids, Packag."}
@STRING{IEEE_J_PMP = "{IEEE} Trans. Parts, Mater., Packag."}
@STRING{IEEE_J_TCAD = "{IEEE} J. Technol. Comput. Aided Design"}
@STRING{IEEE_J_CAD = "{IEEE} Trans. Comput.-Aided Design Integr. Circuits Syst."}
@STRING{IEEE_J_BD = "{IEEE} Trans. Big Data"}
@STRING{IEEE_J_IFS = "{IEEE} Trans. Inf. Forensics Security"}
@STRING{IEEE_J_IT = "{IEEE} Trans. Inf. Theory"}
@STRING{IEEE_J_KDE = "{IEEE} Trans. Knowl. Data Eng."}
@STRING{IEEE_J_CAL = "{IEEE} Comput. Archit. Lett."}
@STRING{IEEE_J_ES = "{IEEE} Embedded Syst. Lett."}
@STRING{IEEE_J_IOT = "{IEEE} Internet Things J."}
@STRING{IEEE_J_XCDC = "{IEEE} J. Explor. Solid-State Computat. Devices Circuits"}
@STRING{IEEE_J_MMCT = "{IEEE} J. Multiscale and Multiphys. Comput. Techn."}
@STRING{IEEE_J_SUSC = "{IEEE} Sustain. Comput."}
@STRING{IEEE_J_CC = "{IEEE} Trans. on Cloud Comput."}
@STRING{IEEE_J_CSS = "{IEEE} Trans. Comput. Social Syst."}
@STRING{IEEE_J_C = "{IEEE} Trans. Comput."}
@STRING{IEEE_J_CNS = "{IEEE} Trans. Control Netw. Syst."}
@STRING{IEEE_J_DSC = "{IEEE} Trans. Depend. Sec. Comput."}
@STRING{IEEE_J_ECOMP = "{IEEE} Trans. Electron. Comput."}
@STRING{IEEE_J_ETC = "{IEEE} Trans. Emerg. Topics Comput."}
@STRING{IEEE_J_EVC = "{IEEE} Trans. Evol. Comput."}
@STRING{IEEE_J_FUZZ = "{IEEE} Trans. Fuzzy Syst."}
@STRING{IEEE_J_MC = "{IEEE} Trans. Mobile Comput."}
@STRING{IEEE_J_MSCS = "{IEEE} Trans. Multi-Scale Comput. Syst."}
@STRING{IEEE_J_NET = "{IEEE/ACM} Trans. Netw."}
@STRING{IEEE_J_NSE = "{IEEE} Trans. Netw. Sci. Eng."}
@STRING{IEEE_J_NSM = "{IEEE} Trans. Netw. Service Manag."}
@STRING{IEEE_J_NN = "{IEEE} Trans. Neural Netw."}
@STRING{IEEE_J_NNLS = "{IEEE} Trans. Neural Netw. Learn. Syst."}
@STRING{IEEE_J_PDS = "{IEEE} Trans. Parallel Distrib. Syst."}
@STRING{IEEE_J_SC = "{IEEE} Trans. Serv. Comput."}
@STRING{IEEE_J_SIPN = "{IEEE} Trans. Signal Inf. Process. Netw."}
@STRING{IEEE_J_SE = "{IEEE} Trans. Softw. Eng."}
@STRING{IEEE_J_JDT = "{IEEE/OSA} J. Display Technol."}
@STRING{IEEE_J_IP = "{IEEE} Trans. Image Process."}
@STRING{IEEE_J_MM = "{IEEE} Trans. Multimedia"}
@STRING{IEEE_J_VCG = "{IEEE} Trans. Vis. Comput. Graphics"}
@STRING{IEEE_J_JAS = "{IEEE/CAA} J. Autom. Sinica"}
@STRING{IEEE_J_JRA = "{IEEE} J. Robot. Autom."}
@STRING{IEEE_J_AFFC = "{IEEE} Trans. Affect. Comput."}
@STRING{IEEE_J_ASE = "{IEEE} Trans. Autom. Sci. Eng."}
@STRING{IEEE_J_AMD = "{IEEE} Trans. Auton. Mental Develop."}
@STRING{IEEE_J_CCN = "{IEEE} Trans. on Cogn. Commun. Netw."}
@STRING{IEEE_J_CDS = "{IEEE} Trans. Cogn. Develop. Syst."}
@STRING{IEEE_J_CIAIG = "{IEEE} Trans. Comput. Intell. {AI} in Games"}
@STRING{IEEE_J_CYB = "{IEEE} Trans. Cybern."}
@STRING{IEEE_J_H = "{IEEE} Trans. Haptics"}
@STRING{IEEE_J_HFE = "{IEEE} Trans. Hum. Factors Electron."}
@STRING{IEEE_J_HMS = "{IEEE} Trans. Human-Mach. Syst."}
@STRING{IEEE_J_MMS = "{IEEE} Trans. Man-Mach. Syst."}
@STRING{IEEE_J_PAMI = "{IEEE} Trans. Pattern Anal. Mach. Intell."}
@STRING{IEEE_J_RA = "{IEEE} Trans. Robot. Autom."}
@STRING{IEEE_J_RAL = "{IEEE} Robot. Autom. Lett."}
@STRING{IEEE_J_RO = "{IEEE} Trans. Robot."}
@STRING{IEEE_J_SMC = "{IEEE} Trans. Syst., Man, Cybern."}
@STRING{IEEE_J_SMCA = "{IEEE} Trans. Syst., Man, Cybern. {A}"}
@STRING{IEEE_J_SMCB = "{IEEE} Trans. Syst., Man, Cybern. {B}"}
@STRING{IEEE_J_SMCC = "{IEEE} Trans. Syst., Man, Cybern. {C}"}
@STRING{IEEE_J_SMCS = "{IEEE} Trans. Syst., Man, Cybern., Syst."}
@STRING{IEEE_J_SSC = "{IEEE} Trans. Syst. Sci. Cybern."}
@STRING{IEEE_J_GRSL = "{IEEE} Geosci. Remote Sens. Lett."}
@STRING{IEEE_J_GE = "{IEEE} Trans. Geosci. Electron."}
@STRING{IEEE_J_GRS = "{IEEE} Trans. Geosci. Remote Sens."}
@STRING{IEEE_J_OE = "{IEEE} J. Ocean. Eng."}
@STRING{IEEE_J_STARS = "{IEEE} J. Sel. Topics Appl. Earth Observ. Remote Sens."}
@STRING{IEEE_J_CJECE = "Canadian J. Elect. Comput. Eng."}
@STRING{IEEE_J_PROC = "Proc. {IEEE}"}
@STRING{IEEE_J_RITA = "{IEEE} Revista Iberoamericana de Technolog{\'{i}}as del Aprendizaje"}
@STRING{IEEE_J_EDU = "{IEEE} Trans. Educ."}
@STRING{IEEE_J_EM = "{IEEE} Trans. Eng. Manag."}
@STRING{IEEE_J_EWS = "{IEEE} Trans. Eng. Writing Speech"}
@STRING{IEEE_J_LT = "{IEEE} Trans. Learn. Technol."}
@STRING{IEEE_J_PC = "{IEEE} Trans. Prof. Commun."}
@STRING{IEEE_J_AWPL = "{IEEE} Antennas Wireless Propag. Lett."}
@STRING{IEEE_J_MAGL = "{IEEE} Magn. Lett."}
@STRING{IEEE_J_MGWL = "{IEEE} Microw. Guided Wave Lett."}
@STRING{IEEE_J_MWCL = "{IEEE} Microw. Wireless Compon. Lett."}
@STRING{IEEE_J_RFIC = "{IEEE} {RFIC} J."}
@STRING{IEEE_J_RFID = "{IEEE} {RFID} J."}
@STRING{IEEE_J_AP = "{IEEE} Trans. Antennas Propag."}
@STRING{IEEE_J_EMC = "{IEEE} Trans. Electromagn. Compat."}
@STRING{IEEE_J_MAG = "{IEEE} Trans. Magn."}
@STRING{IEEE_J_MTT = "{IEEE} Trans. Microw. Theory Techn."}
@STRING{IEEE_J_RFI = "{IEEE} Trans. Radio Freq. Interference"}
@STRING{IEEE_J_TTHZ = "{IEEE} Trans. {THz} Sci. Technol."}
@STRING{IEEE_J_TJMJ = "{IEEE} Transl. J. Magn. Jpn."}
@STRING{IEEE_J_PHOT = "{IEEE} J. Photovolt."}
@STRING{IEEE_J_PEL = "{IEEE} Power Electron. Lett."}
@STRING{IEEE_J_PETS = "{IEEE} Power Energy Technol. Syst. J."}
@STRING{IEEE_J_ESTPE = "{IEEE} Trans. Emerg. Sel. Topics Power Electron."}
@STRING{IEEE_J_EC = "{IEEE} Trans. Energy Convers."}
@STRING{IEEE_J_PWRAS = "{IEEE} Trans. Power App. Syst."}
@STRING{IEEE_J_PWRD = "{IEEE} Trans. Power Del."}
@STRING{IEEE_J_PWRE = "{IEEE} Trans. Power Electron."}
@STRING{IEEE_J_PWRS = "{IEEE} Trans. Power Syst."}
@STRING{IEEE_J_SG = "{IEEE} Trans. Smart Grid"}
@STRING{IEEE_J_STE = "{IEEE} Trans. Sustain. Energy"}
@STRING{IEEE_J_PSE = "{IEEE} J. Product Safety Eng."}
@STRING{IEEE_J_APPIND = "{IEEE} Trans. Appl. Ind."}
@STRING{IEEE_J_BC = "{IEEE} Trans. Broadcast."}
@STRING{IEEE_J_BCTV = "{IEEE} Trans. Broadcast Television Receivers"}
@STRING{IEEE_J_CE = "{IEEE} Trans. Consum. Electron."}
@STRING{IEEE_J_IE = "{IEEE} Trans. Ind. Electron."}
@STRING{IEEE_J_IECI = "{IEEE} Trans. Ind. Electron. Contr. Instrum."}
@STRING{IEEE_J_IA = "{IEEE} Trans. Ind. Appl."}
@STRING{IEEE_J_IGA = "{IEEE} Trans. Ind. Gen. Appl."}
@STRING{IEEE_J_IINF = "{IEEE} Trans. Ind. Informat."}
@STRING{IEEE_J_IM = "{IEEE} Trans. Instrum. Meas."}
@STRING{IEEE_J_JEM = "{IEEE/TMS} J. Electron. Mater."}
@STRING{IEEE_J_DEI = "{IEEE} Trans. Dielectr. Electr. Insul."}
@STRING{IEEE_J_EI = "{IEEE} Trans. Electr. Insul."}
@STRING{IEEE_J_MEMS = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MEMSI = "J. Microelectromech. Syst."}
@STRING{IEEE_J_MECH = "{IEEE/ASME} Trans. Mechatronics"}
@STRING{IEEE_J_BHI = "{IEEE} J. Biomed. Health Inform."}
@STRING{IEEE_J_TEHM = "{IEEE} J. Transl. Eng. Health Med."}
@STRING{IEEE_J_LS = "{IEEE} Life Sci. Lett."}
@STRING{IEEE_J_RBME = "{IEEE} Rev. Biomed. Eng."}
@STRING{IEEE_J_BCAS = "{IEEE} Trans. Biomed. Circuits Syst."}
@STRING{IEEE_J_BMELC = "{IEEE} Trans. Bio-Med. Electron."}
@STRING{IEEE_J_BME = "{IEEE} Trans. Biomed. Eng."}
@STRING{IEEE_J_B-ME = "{IEEE} Trans. Bio-Med. Eng."}
@STRING{IEEE_J_CBB = "{IEEE/ACM} Trans. Comput. Biol. Bioinformatics"}
@STRING{IEEE_J_ITBM = "{IEEE} Trans. Inf. Technol. Biomed."}
@STRING{IEEE_J_ME = "{IEEE} Trans. Med. Electron."}
@STRING{IEEE_J_MI = "{IEEE} Trans. Med. Imag."}
@STRING{IEEE_J_MBSC = "{IEEE} Trans. Mol. Biol. Multi-Scale Commun."}
@STRING{IEEE_J_NB = "{IEEE} Trans. Nanobiosci."}
@STRING{IEEE_J_NSRE = "{IEEE} Trans. Neural Syst. Rehabil. Eng."}
@STRING{IEEE_J_RE = "{IEEE} Trans. Rehabil. Eng."}
@STRING{IEEE_J_JLT = "J. Lightw. Technol."}
@STRING{IEEE_J_OCN = "{IEEE} J. Opt. Commun. Netw."}
@STRING{IEEE_J_PJ = "{IEEE} Photon. J."}
@STRING{IEEE_J_PTL = "{IEEE} Photon. Technol. Lett."}
@STRING{IEEE_J_EDL = "{IEEE} Electron Device Lett."}
@STRING{IEEE_J_EDS = "{IEEE} J. Electron Devices Soc."}
@STRING{IEEE_J_JQE = "{IEEE} J. Quantum Electron."}
@STRING{IEEE_J_JSTQE = "{IEEE} J. Sel. Topics Quantum Electron."}
@STRING{IEEE_J_ENANO = "{IEEE} Nanotechnol. Express"}
@STRING{IEEE_J_ED = "{IEEE} Trans. Electron Devices"}
@STRING{IEEE_J_NANO = "{IEEE} Trans. Nanotechnol."}
@STRING{IEEE_J_NS = "{IEEE} Trans. Nucl. Sci."}
@STRING{IEEE_J_PS = "{IEEE} Trans. Plasma Sci."}
@STRING{IEEE_J_DMR = "{IEEE} Trans. Device Mater. Rel."}
@STRING{IEEE_J_R = "{IEEE} Trans. Rel."}
@STRING{IEEE_J_ESSL = "{IEEE/ECS} Electrochem. Solid-State Lett."}
@STRING{IEEE_J_JSSC = "{IEEE} J. Solid-State Circuits"}
@STRING{IEEE_J_ASC = "{IEEE} Trans. Appl. Supercond."}
@STRING{IEEE_J_SM = "{IEEE} Trans. Semicond. Manuf."}
@STRING{IEEE_J_SENSOR = "{IEEE} Sensors J."}
@STRING{IEEE_J_VLSI = "{IEEE} Trans. {VLSI} Syst."}
@STRING{IEEE_O_ACC = "{IEEE} Access"}
@STRING{IEEE_M_AES = "{IEEE} Aerosp. Electron. Syst. Mag."}
@STRING{IEEE_M_HIST = "{IEEE} Ann. Hist. Comput."}
@STRING{IEEE_M_AP = "{IEEE} Antennas Propag. Mag."}
@STRING{IEEE_M_ASSP = "{IEEE} {ASSP} Mag."}
@STRING{IEEE_M_CHINAC = "China Commun."}
@STRING{IEEE_M_CD = "{IEEE} Circuits Devices Mag."}
@STRING{IEEE_M_CAS = "{IEEE} Circuits Syst. Mag."}
@STRING{IEEE_M_COM = "{IEEE} Commun. Mag."}
@STRING{IEEE_M_COMSOC = "{IEEE} Commun. Soc. Mag."}
@STRING{IEEE_O_CSTO = "{IEEE} Commun. Surveys Tuts."}
@STRING{IEEE_M_CIM = "{IEEE} Comput. Intell. Mag."}
@STRING{IEEE_M_CSE = "{IEEE} Comput. Sci. Eng."}
@STRING{IEEE_M_CSEM = "{IEEE} Comput. Sci. Eng. Mag."}
@STRING{IEEE_M_C = "Computer"}
@STRING{IEEE_M_CAP = "{IEEE} Comput. Appl. Power"}
@STRING{IEEE_M_CGA = "{IEEE} Comput. Graph. Appl."}
@STRING{IEEE_M_CONC = "{IEEE} Concurrency"}
@STRING{IEEE_M_CS = "{IEEE} Control Syst. Mag."}
@STRING{IEEE_M_DT = "{IEEE} Des. Test"}
@STRING{IEEE_M_DTC = "{IEEE} Des. Test. Comput."}
@STRING{IEEE_O_DSO = "{IEEE} Distrib. Syst. Online"}
@STRING{IEEE_M_EI = "{IEEE} Electr. Insul. Mag."}
@STRING{IEEE_M_ETF = "{IEEE} Electrific. Mag."}
@STRING{IEEE_M_EMC = "{IEEE} Electromagn. Compat."}
@STRING{IEEE_M_ETR = "{IEEE} ElectroTechnol. Rev."}
@STRING{IEEE_M_EMR = "{IEEE} Eng. Manag. Rev."}
@STRING{IEEE_M_EMB = "{IEEE} Eng. Med. Biol. Mag."}
@STRING{IEEE_M_EXP = "{IEEE} Expert"}
@STRING{IEEE_M_GRS = "{IEEE} Geosci. Remote Sens. Mag."}
@STRING{IEEE_M_IA = "{IEEE} Ind. Appl. Mag."}
@STRING{IEEE_M_IE = "{IEEE} Ind. Electron. Mag."}
@STRING{IEEE_M_IM = "{IEEE} Instrum. Meas. Mag."}
@STRING{IEEE_M_IS = "{IEEE} Intell. Syst."}
@STRING{IEEE_M_ITS = "{IEEE} Intell. Transp. Syst. Mag."}
@STRING{IEEE_M_IC = "{IEEE} Internet Comput."}
@STRING{IEEE_M_ITP = "{IEEE} {IT} Prof."}
@STRING{IEEE_M_MICRO = "{IEEE} Micro"}
@STRING{IEEE_M_MW = "{IEEE} Microw. Mag."}
@STRING{IEEE_M_MM = "{IEEE} Multimedia"}
@STRING{IEEE_M_NANO = "{IEEE} Nanotechnol. Mag."}
@STRING{IEEE_M_NET = "{IEEE} Netw."}
@STRING{IEEE_M_PCOM = "{IEEE} Personal Commun. Mag."}
@STRING{IEEE_M_PVC = "{IEEE} Pervasive Comput."}
@STRING{IEEE_M_POT = "{IEEE} Potentials"}
@STRING{IEEE_M_PEL = "{IEEE} Power Electron. Mag."}
@STRING{IEEE_M_PE = "{IEEE} Power Energy Mag."}
@STRING{IEEE_M_PER = "{IEEE} Power Eng. Rev."}
@STRING{IEEE_M_PULSE = "{IEEE} Pulse"}
@STRING{IEEE_M_RA = "{IEEE} Robot. Autom. Mag."}
@STRING{IEEE_M_SAP = "{IEEE} Security Privacy"}
@STRING{IEEE_M_SP = "{IEEE} Signal Process. Mag."}
@STRING{IEEE_M_S = "{IEEE} Softw."}
@STRING{IEEE_M_SSC = "{IEEE} Solid-State Circuits Mag."}
@STRING{IEEE_M_SPECT = "{IEEE} Spectr."}
@STRING{IEEE_M_SMC = "{IEEE} Syst., Man, Cybern. Mag."}
@STRING{IEEE_M_TS = "{IEEE} Technol. Soc. Mag."}
@STRING{IEEE_M_VT = "{IEEE} Veh. Technol. Mag."}
@STRING{IEEE_M_WC = "{IEEE} Wireless Commun."}
@STRING{IEEE_M_TODAY = "Today's Engineer"}

